Prioritizing and Scheduling Conferences for Metadata Harvesting in dblp

Maintaining literature databases and online bibliographies is a core responsibility of metadata aggregators such as digital libraries. In the process of monitoring all the available data sources the question arises which data source should be prioritized. Based on a broad definition of information quality we are looking for different ways to find the best fitting and most promising conference candidates to harvest next. We evaluate different conference ranking features by using a pseudo-relevance assessment and a component-based evaluation of our approach.

==> input/notation.tex <==
Dates $d=(m,y)$ are represented as pairs of a month $m$ (numeric or symbolic?) and a year $y$. The difference of two dates is the number of months between the dates. Adding $\delta$ months to a date yields a date that is $\delta$ months later. $year(d)$ yields the year, $month(d)$ yields the month of date $d$.

Set of conferences $C$ to consider.

Conference (JCDL, SIGIR, etc.) $c\in C$ is a set of conference events (or short events) $E(c)=\{e_1,\ldots,e_n\}$ stored in the bibliography.

For each event $e$, we may know
\begin{itemize}
\item the date $d(e)$ of the first day of the event
\item its release date $r(e)$ of its proceedings % ggf. approximiert durch die Aufnahme in die Bibliographie
\item its insert delay $\delta(e):=d(e)-r(e)$ % stimmt das? oder ist das publication delay?
\item its location $l(e)$ representing the country where the event took place
\item its number of papers $p(e)$
\item its number of distinct authors $a(e)$ % ggf. für prominence
\item its number of incoming citations $c(e,y)$ until year $y$, i.e., the number of times a paper that appeared in $e$ is cited from a paper that appeared in a year not larger than $y$.
\end{itemize}

For a conference $c$ with its events $E(c)$, we assume that the events in $E(c)$ are ordered in increasing consider of their date, i.e., the last event in $E(c)$ is the most recent one. $last(c)$ denotes the most recent event of $c$.

We then compute the following features for $c$:
\begin{itemize}
\item its characteristic interval $\delta_{year}(c)$ as the median of distance of the years of the six most recent subsequent events in $E(c)$ (or of all events if $c$ has less than six events)\\
median of $\{year(d(e_{i+1})-year(d(e_{i})|i=max(1,|E(c)|-6)\ldots|E(c)|-1\}$ if $|E(c)|>1$, 0 otherwise % gefällt mir noch nicht, aber wenn man das formal präzise aufschreibt, wird's unübersichtlich; Konferenzen, die mehr als einmal im Jahr stattfinden?
\item its expected month $m(c)$ as the average month $month(d(e))$ of the five most recent events in $E(c)$ % wie auch immer man das ausrechnet; Monate sind Ordinale, da kann man keinen Durchschnitt bestimmen - was ist bei Konferenzen, die mal im Dezember und mal im Januar stattfinden?
\item its characteristic delay $\delta_{month}(c)$ as the median of the delays of the five most recent events in $E(c)$ (or of all events if $c$ has less than five events) % s.o. für die präzise formale Beschreibung
\item its rating $r(c)$, which is a numeric value where larger values indicate higher rating. Can be taken from external source such as CORE or ERA
\item its internationality $i(c):=|\cup_{e\in E(c)}l(c)|$ as the number of distinct countries where the conference has taken place
\item its number of incoming citations $c(c,y)$ until year $y$ as $c(c,y):=\sum_{e\in E(c) \wedge year(d(e))\leq y}c(e,y)$
\end{itemize}

The expected date E(c) of the next event of $c$ is computed as $$E(c):=d(last(c))+12*I(c)+\delta(c)$$

Now rank conferences to add in month $m$ and year $y$; exclude conference where $E(c)$ is later
\begin{itemize}
\item conference rating: $w_r(c):=\frac{r(c)}{max_Cr(c)}$

\item internationality: $w_i(c):= \frac{i(c)}{max_Ci(c)}$

\item discontinued conferences % w_d: welches Jahr ist hier gemeint, Konferenzjahr oder Publikationsjahr?

\item incoming citations: average number of incoming citations up to year $y-1$ per paper published in $c$
$w_c:=\frac{c(c,y-1)}{\sum_{ e\in E(c) \wedge year(d(e))<y}p(e)}$

\end{itemize}

